Satellite-Terrestrial Quantum Networks and the Global Quantum Internet

This paper will explore the design and implementation of quantum networks in space integrated with quantum networks on Earth. We propose a three-layer approach, involving GEO and LEO satellites integrated with terrestrial ground stations. We first analyze the channel conditions between the three layers, and then highlight the key role of LEO satellites in the integrated space-terrestrial system - namely the source of entanglement distribution between specified terrestrial stations via direct downlink quantum-optical channels. The GEO satellites in the considered system are used primarily as coordination stations, managing and directing the LEO satellites regarding the positioning and timing of entanglement distribution. Complexity, in the form of entanglement distillation and quantum-state correction, is concentrated at the terrestrial stations, and teleportation is used as the primary quantum channel in the LEO uplinks and the inter-terrestrial channels. Although our designs are futuristic in that they assume limited quantum memory at the transceivers, we also discuss some near-term uses of our network in which no quantum memory is available.

==> WINS-LatexInclusion/Catechism/WINS-Catechism.tex <==
%----------------------------------------------------------------------------------------%
%                                   W I N S   C a t e c h i s m                              %
%----------------------------------------------------------------------------------------%
\section*{WINS\,Lab Research Paper Catechism}
\vspace{-1.5mm}
\centerline{\footnotesize\emph{(Adapted from George Heilmeier)}}

\vspace{0.5cm} 

Please \emph{think} about the following questions carefully and answer them as concisely as you can before starting to write your manuscript. This will help you sharpening the ideas and improve the writing style. You will also find that you have effectively written the Introduction and Conclusion of the manuscript as soon as you finish answering these questions. It is important that you spend some time on this as the answers to these questions will become the backbone of the manuscript.


\be\itemsep3ex

\item What is the big picture? What is the problem? Why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem: \Problem
	\item[$\diamond$] The Difficulty: \Difficulty
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Conventional Approaches: \ConventionalApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous works. Provide references (use the first three alphabets of the authors' last names, capitalizing the first letter each, followed by ``:'' and two-digit year, as per convention in our database, e.g., BenShoSmoTha:02 in WINS-Quantum.bib).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\diamond$] \FundamentalQ
	\item[$\diamond$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts. In writing the fundamental questions, try to start with different words such as ``what", ``how'', ``why''.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
		\be
		\item[$\circ$] \Goals 
		\ee	
	\ei
				
\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{This is related to the main breakthrough of the paper.}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{What is the magic sauce you put together for unleashing the advocated idea.}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: 
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] \HLContribution
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
		\mysubsubnote{Avoid the excessive use of ``we''. Instead of using ``we'', you can start with verb/noun like ``present the/presentation of \ldots'', ``develop a/development of'', ``characterize the/characterization of'', ``quantify the/quantification of''.}
	\ei

\item Which are the research methodologies?
	\bi
	\item[$\diamond$] The Methodologies: \Methodologies
	\ei

\item How is the approach verified?
	\bi
	\item[$\diamond$] The Verification: \Verification
	\item[ ] \mysubsubnote{In responding, describe which figures of merit are used and how the results are confirmed.}
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned? What are the surprising results?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned: \ConclusiveLesson
	\item[$\diamond$] The Surprising Results: \SurprisingResults
	%\item[ ] \mysubsubnote{These two items will form the Conclusion, so think about what are the take away messages.}
	\ei

\item What are the intellectual merits? What is the impact; what are the benefits to a broader community?
	\bi
	\item[$\diamond$] The Intellectual Merits: \IntellectualMerits
	\item[$\diamond$] The Impact/Benefits: \BroaderImpacts
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures: \Disclosures
	\item[$\diamond$] Sources: \Sources
	\ei

\item What are the key references?
	\bi
	\item[$\diamond$] Key References: \KeyReferences
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
	\ei

\ee


==> Work-In-Progress/LatexInclusion/Local-Acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	\newacro{<acronym>}[<short name>]{<full name>}
%
% 	House style: 
% 		enter the acronym alphabetically
% 		always use capital letter when calling the acronym even if you want to show it lower case
%
% 	For example, we always call \ac{LOT} even if it appears as LoT in the manuscript through the following definition
%
%	 \newacro{LOT}[LoT]{Localization-of-Things}
%
%	Add new Acronym entries here.
%	Migrate them to "WINS-Acronym.tex" only when the project/paper is completed.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newacro{COT}[COT]{counterfactual oblivious telecomputation}
\newacro{CUO}[CUO]{controlled unitary operation}
\newacro{DQC}[DQC]{distributed quantum computing}
\newacro{DEP}[DEP]{discrimination error probability}
\newacro{PACS}[PACS]{photon-added coherent state}
\newacro{PAGS}[PAGS]{photon-added Gaussian state}
\newacro{POVM}[POVM]{positive operator-valued measure}
\newacro{PSK}[PSK]{phase shift keying}
\newacro{PVQS}[PVQS]{photon-varied quantum state}
\newacro{QAM}[QAM]{quadrature amplitude modulation}
\newacro{QKD}[QKD]{quantum key distribution}
\newacro{SRM}[SRM]{square root measurement}






==> Work-In-Progress/LatexInclusion/Local-Catechism-Def.tex <==
%----------------------------------------------------------------------------------------%
%                         M y     C a t e c h i s m    D e f i n i t i o n s              %
%.              (directly fill-in catechism, introduction, and conclusion)    %
%----------------------------------------------------------------------------------------%

\newcommand{\BigPicture}{Describe the big picture of the problem.
}

\newcommand{\Problem}{Present the problem.
}

\newcommand{\Difficulty}{Present the difficulties of the problem.
}

\newcommand{\ConventionalApproach}{Report the conventional approach before the basic idea of the paper came out.
}

\newcommand{\SOADeficiency}{Narrate the state-of-the-art related to the idea with an indication of its deficiency.
}

\newcommand{\FundamentalQ}{The fundamental questions related to \ldots\ are \ldots\ and \ldots
}

\newcommand{\EnablingA}{The answers to these questions will enable \ldots
}

\newcommand{\Goals}{The goals of this paper are \ldots\  and \ldots. We aim to \ldots
}

\newcommand{\Advocacy}{We advocate \ldots, a new paradigm in which \ldots. The key idea is \ldots.  Our view is \ldots. We believe that \ldots
}

\newcommand{\AdvocacyTwo}{
}

\newcommand{\ReasonSuccess}{We believe that \ldots
}

\newcommand{\ReasonSuccessTwo}{
}

\newcommand{\HLContribution}{In this paper, \ldots\ describe what we do at a high level \ldots 
}

\newcommand{\KeyContribution}{The key contributions of this paper are as follows:
			\begin{itemize}
			\item[$\bullet$] We develop a framework for \ldots; We establish foundation for \ldots; We determine the fundamental limits of \ldots; 
			\item[$\bullet$] We introduce the concepts of \ldots;  We put forth the notion of \ldots; We propose a new model \ldots; 
			\item[$\bullet$] We characterize \ldots; We design \ldots; We analyze\ldots; We derive \ldots; We prove that \ldots; We show that \ldots; We quantify the \ldots; 
			\item[$\bullet$] Our analysis reveals the innate connection between A and B \ldots; We provide insights into the essence of \ldots; 
						We provide a complete probabilistic characterization of \ldots; We provide guidelines for \ldots
			\end{itemize}
}

\newcommand{\Methodologies}{Describe the methodology/approach (analysis, simulation, experimentation, or combination of them) used to solve/overcome the problem described in Question~1.
}

\newcommand{\Verification}{Describe how the contributions described in Question~6 are verified. Present the case-studies considered and the performance metrics adopted in the paper.
}

\newcommand{\ConclusiveVision}{Clearly articulate the new vision, new perspective, new technical idea, and new view provided by the paper.
}

\newcommand{\ConclusiveLesson}{Provide take away messages. Recount the lessons learned as a result of the hard work described in this paper.
}

\newcommand{\SurprisingResults}{Describe the surprising results in the paper and corresponding useful insights.
}

\newcommand{\IntellectualMerits}{Describe intellectual merits of the paper.
}

\newcommand{\BroaderImpacts}{End with the impact/benefits of the results to a broader community.
}

\newcommand{\Disclosures}{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).
}

\newcommand{\Sources}{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).
}

\newcommand{\KeyReferences}{
}

==> Work-In-Progress/LatexInclusion/Local-Definitions.tex <==
% put latex definitions specific to your paper here.
% For example: \newcommand{\samplesize}{n}


%---------------------%
% Symbols             %
%---------------------%

%---------------------%
% References        %
%---------------------%
%\newcommand{\fig}[1]{Fig.~\ref{#1}}
%\newcommand{\sect}[1]{Sec.~\ref{#1}}
%\newcommand{\apd}[1]{Appendix~\ref{#1}}
%\newcommand{\eq}[1]{(\ref{#1})}


%--------------------------------------------------------------%
% Define quick color commands 		          %
%--------------------------------------------------------------%

\providecommand{\cbl}{\textcolor{blue}}
\providecommand{\crd}{\textcolor{red}}



==> Work-In-Progress/Sections/EDFL.tex <==
\textcolor{blue}{\it This section presents distribution of entanglement with finite lifetime.}

==> Work-In-Progress/Sections/Introduction.tex <==
\textcolor{blue}{\it This is the introduction.}

%\mynote{Answer to Q1}
\mysubnote{Big Picture} %\BigPicture
\IEEEPARstart{Q}{uantum networks}  
 
\mysubnote{Problem} %\Problem
\mysubnote{Difficulty} %\Difficulty

%\mynote{Answer to Q2}
\mysubnote{Conventional Approaches} %\ConventionalApproach

\mysubnote{SVE and Deficiencies} %\SOADeficiency

%\mynote{Answer to Q3}
\mysubnote{Fundamental Questions} %\FundamentalQ
\mysubnote{What Answers Enables} %\EnablingA
%\mynote{Answer to Q4}
\mysubnote{The Goals} %\Goals
%\mynote{Answer to Q5}
%\mysubnote{Reasons of Success}\ReasonSuccess
\mysubnote{New View/Idea} %\Advocacy

%\mynote{Answer to Q6}
\mysubnote{High-Level Contribution} %\HLContribution
\mysubnote{Key contributions} %\KeyContribution

==> Work-In-Progress/Sections/QSD.tex <==
%\textcolor{blue}{\it This section presents quantum state design and discrimination for satellite-terrestrial quantum networks.}
\newcommand{\qstate}{\M{\Xi}}
\newcommand{\qstateRV}{\RM{\Xi}}
\newcommand{\qmeas}{\M{\Pi}}
\newcommand{\rhoRV}{\qstateRV}
\renewcommand{\rho}{\qstate}

Thus far we have avoided any detailed technical discussions on the various aspects of the GCI - this may lead to a false impression on the reader's part as to the complexity of such a network, and the amount of detailed ongoing research that  is being carried out in regard to various aspects of the GCI. The reality is the GCI will involve the deployment many complicated quantum tasks. In  an article such as this, it is impossible to discuss all such tasks. However, it is perhaps worthwhile to end with some detailed discussion on at least one of these tasks so as to provide some insight into the complexities that will underpin the GCI - and the nature of related ongoing quantum technology research. To this end, we choose \Ac{QSD} as the topic of our last discussion - a task that
 aims to identify an unknown state among a set of quantum states \cite{Hel:B76,Hol:73,YueKenLax:75}, and is an essential component (building block) for several \ac{QN} applications including quantum communications, %\cite{HelLiuGor:70,Car:B15,Lin:20}, 
sensing, %\cite{DegReiCap:17,GioLloMac:04b,Par:07}, 
illumination, %\cite{Llo:08,TanErkGioGuhLloMacPirSha:08,LopRuoDegOliBriGen:13}, 
cryptography, % \cite{GisRibTitZbi:02,ScaBecCerDusLutPee:09,GueChiCon:18}, 
control, %quantum networks \cite{ChiDarMauPer:09,Kim:08,DaiPenWin:J20a}, 
and computing \cite{ref1}. \Ac{QSD} is of particular importance in the CV realm. 
% \cite{NieChu:B10,CleEkeMacMos:98,BerHerHil:03}. 
The quantum \ac{DEP} depends on the set of states and measurement used.
%(see Fig.~\ref{fig:qsd}). 
%In particular, continuous-variable quantum states have been  considered in quantum optics for describing the electromagnetic field in quantum domain. Continuous-variable quantum states can be efficiently prepared, modified, and measured. Therefore, designing quantum states for improving \ac{QSD} capabilities is essential for operation of satellite-terrestrial quantum networks.

%\begin{figure}[!t]
%\vspace{0.05cm}
%\centering
%\includegraphics[scale=0.98]{Figures/QSD.eps}
%\caption{Illustration of binary \ac{QSD} with \acp{PACS}\cite{GueWinChiCon:J20}: hypotheses $H_0$ and $H_1$ are associated with the density matrix of two quantum state and decision $\hat{H}$ is taken based on a binary \ac{POVM} \{\qmeas_0, \qmeas_1\}$.}
%\label{fig:qsd}
%\end{figure}

It has been recently demonstrated in \cite{GueWinChiCon:J20} that exploiting non-coherent (i.e., non-classical) states can provide performance gain in terms of \ac{DEP}. In particular, \acp{PACS} has been characterized in terms of Fock basis, Wigner $W$-function, Glauber–Sudarshan $P$-function,and Husimi–Kano $Q$-function, when affected by thermal noise during state preparation. Based on such characterization, \acp{PACS} are designed to improve the \ac{QSD} performance with respect to coherent states both with ideal quantum receiver and with classical receiver accounting for decoherence and losses. Such properties and state design capabilities have been extended and generalized  in \cite{GueWinCon:J23} to a wider class of non-coherent states, namely \acp{PVQS}, which generalize non-classical states that are obtained either via photon addition or photon subtraction operations. Since Gaussian states lack some desirable properties (e.g.,Wigner function negativity) for unleashing the quantum superiority in various applications \cite{AdeRagLee:14}, it is important to identify and characterize new classes of non-Gaussian states that offer performance gain, yet are easy to prepare,in quantum systems and networks. 

The unified characterization of \ac{PVQS} enables the design and analysis of satellite-terrestrial quantum systems and networks that exploit non-Gaussian properties. 
%os states carrying information 
For example, the use of non-Gaussian \acp{PAGS} for quantum \ac{QAM} communications has been presented  in \cite{GiaWinCon:C23b}, showing how to construct arbitrary \ac{QAM} constellations of \acp{PAGS}.
%(see Fig.~\ref{fig:PSKsubconstellation}). 
The performance gain using \acp{PAGS} with engineered displacement, squeezing, and photon variation is quantified when a \ac{SRM} receiver is employed, and compared with the one provided by conventional coherent states.

The design of a quantum state is  important not only for \ac{QSD}-based applications, but also for enabling communication security via \ac{QKD} protocols. \ac{QKD} protocols suffer from non-ideal sources and, therefore, decoy-state protocols were proposed \cite{LoMaChe:05}. The design of quantum decoy states for \ac{QKD} (number of photon-addition operations, displacing parameter, and squeezing parameter with respect to noise level in state preparation) has been shown recently \cite{GiaWinCon:C23} and is particularly important in the presence of non-ideal sources at Earth or Satellite emitters. Thus, engineering of non-ideal sources is essential for improving the performance of the \ac{QKD} decoy-state protocols in integrated satellite-terrestrial quantum networks.

%\begin{figure}[t!]
%	\centering
%	\resizebox{0.7\columnwidth}{!}{\includegraphics{Figures/Constellation.pdf}}
%	\caption{Representation of the quaternary \ac{PSK} sub-constellation from which any arbitrary $M$-\ac{QAM} constellation can be build \cite{GiaWinCon:C23b}. The reference state is depicted as the ellipse (contour plot of the associated Wigner function) in the first quadrant and with center determined by the thick blue vector, which represents the displacement in polar coordinates. The ellipse is tilted according to the squeezing parameter. The remaining states are obtained from an anticlockwise rotation.}
%\label{fig:PSKsubconstellation}
%\end{figure}






==> Work-In-Progress/Sections/Qnoise.tex <==
\textcolor{blue}{\it This section establishes models for quantum channel and noise in satellite-terrestrial quantum networks.}

==> Work-In-Progress/Sections/STQN-scenarios.tex <==
\textcolor{blue}{\it This section describes integrated satellite-terrestrial quantum networks.}

==> Work-In-Progress/Sections/STQcom.tex <==
\textcolor{blue}{\it This section presents inter-satellite communications, earth-to-satellite communications, and integrated satellite-terrestrial communications in quantum networks.}

